Alignment-Enhanced Decoding:Defending via Token-Level Adaptive Refining of Probability Distributions

Large language models are susceptible to jailbreak attacks, which can result in the generation of harmful content. While prior defenses mitigate these risks by perturbing or inspecting inputs, they ignore competing objectives, the underlying cause of alignment failures. In this paper, we propose Alignment-Enhanced Decoding (AED), a novel defense that employs adaptive decoding to address the root causes of jailbreak issues. We first define the Competitive Index to quantify alignment failures and utilize feedback from self-evaluation to compute post-alignment logits. Then, AED adaptively combines AED and post-alignment logits with the original logits to obtain harmless and helpful distributions. Consequently, our method enhances safety alignment while maintaining helpfulness. We conduct experiments across five models and four common jailbreaks, with the results validating the effectiveness of our approach. Code is available at https://github.com/GIGABaozi/AED.git.

==> tables/different_queries.tex <==
\begin{table}[t!]
\small 
  \centering
  \begin{tabular}{ @{} l|c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}}
        % { c |c c}
        \toprule 
    & w/o Sys Prompt & w/ Sys Prompt  \\ \midrule 
 
    Routine & 96.7\% & 97\%   \\ \midrule
    Jailbreak & 23.5\% & 58.5\%   \\ \bottomrule

  \end{tabular}
    \caption{The table provides the percentage of~\aedindex~lower than \textbf{threshold} under different queries. Obviously, the 
    %200 samples. LLaMa2. GCG
    }
    \caption{The table provides the success rates of routine and jailbreak queries, illustrating the percentage of responses with \aedindex~below a certain threshold. With system prompts, success rates in handling jailbreak queries improve significantly from 23.5\% to 58.5\%, indicating enhanced system robustness. However, there is a slight decrease in the performance on routine queries, from 97\% to 96.7\%, possibly due to the increased complexity introduced by the prompts.}
     \label{tab: different_queries}
% updated with new Hidden_random
\end{table}
